Machine Learning the Phenomenology of COVID-19 From Early Infection Dynamics

We present a robust data-driven machine learning analysis of the COVID-19 pandemic from its early infection dynamics, specifically infection counts over time. The goal is to extract actionable public health insights. These insights include the infectious force, the rate of a mild infection becoming serious, estimates for asymtomatic infections and predictions of new infections over time. We focus on USA data starting from the first confirmed infection on January 20 2020. Our methods reveal significant asymptomatic (hidden) infection, a lag of about 10 days, and we quantitatively confirm that the infectious force is strong with about a 0.14% transition from mild to serious infection. Our methods are efficient, robust and general, being agnostic to the specific virus and applicable to different populations or cohorts.

==> abstract-1.tex <==
We present a data-driven machine learning analysis of COVID-19 from its
  \emph{early} infection dynamics, with the goal of extracting
  actionable public health insights, including predictions for the number of
  new infections over time. We focus on 
  the transmission dynamics in the USA starting from the first confirmed
  infection on January 21 2020. We find that COVID-19 has a strong
  infectious force if left unchecked, with a doubling time of
  under 3 days. However it is not particularly virulent. Our methods
  may be of general interest.


==> intro-1.tex <==
\section{Introduction}
\label{section:intro}

On March 1 on ABC's This Week, US Secretary of Health and Human
Services Alex Azar told host George Stephanopoulos that
asymptomatic spread of COVID-19 is ``not the major driver'' of the spread of
the new coronavirus, a sentiment corroborated on the CDC's website.
Meanwhile other researchers disagreed, for example
Dr. Osterholm, director of the Center for Infectious Disease Research
and Policy at the University of Minnesota and Dr.
Schaffner of the Vanderbilt University Medical School 
and adviser to the CDC (see the CNN article, \cite{CNN2020}).
At the time, there
was clearly no unimodal opinion.
What does the data say?
There is a clear need for generating actionable intelligence on the nature
of a pandemic from \emph{early} and minimal data.

One approach is scenario analysis.
Recently, \cite{Chinazzi2020} used
the Global Epidemic and Mobility Model (GLEAM)
to perform infection scenario analyses on China COVID-19
data, using
a networked meta-population model based on transportation hubs.
A similar model for the US was reported in \cite{TIME2020} where their
web-app predicts from 150,000 to 1.4 million infected cases by April 30,
depending on the intervention level.
Such
complex scenario analysis requires user input such as infection
sites and properties of the contagion. However,
a majority of infection sites may be hidden, especially if asymptomatic
transmission is significant, and the contagion parameters are
\emph{unknown} and 
must be deduced, perhaps using domain expertise.

Data driven approaches are powerful. A long range regression analysis of
COVID-19 out to 2025 on US data using immunological,
epidemiological and seasonal
effects is given in \cite{Kissler2020},
which predicts  recurrent outbreaks.
We also follow a pure data-driven machine learning
approach to understand early dynamics of COVID-19 on the first
54 days of US confirmed infection reports (downloadable from
the European Center For Disease Control).
We address the challenge of real-time data-intelligence from early data.
Our data-approach
is simple, requires minimal data or human input and generates
fast actionable insights.
Is asymptomatic spread significant?
Our data-driven analysis says yes, emphatically.
What are the properties of the contagion,
for example is it unusually virulent? Our analysis says no.

Early data
is both a curse and a blessing.
The curse is that ``early'' implies not
much information, so quantitative models must be simple and robust
to be identifiable from the data.
The blessing is that early data is
a peek at the pandemic as it roams free,
unchecked by public health protocols, for
to learn the true intentions of the lion, you must follow the
beast on the savanna, not in the zoo.
As we will see, much can be learned from early data and
these insights early in the game, that are not based on opinion but data,
are crucial to public health governance.

\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics[width=0.6\textwidth,trim={1cm 6.7cm 1.35cm 6.9cm},clip]{Fig1}};
    \foreach\y/\x[count=\i]in{1/{1/21},10/{2/1},20/{2/10},30/{2/20},40/{3/1},50/{3/10},54/{3/14}}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y-1+2)/(55-0+4)}%xmin=1,xmax=56
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.75,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }

    \foreach\y[count=\i]in{500,1000,1500,2000,2500,2180,2845}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y^(0.75)+6)/(2945^(0.75)+1+12)}%ymin=-1,ymax=2945^0.75
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.7,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
      }
    
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.06*(F.south)-0.06*(F.north)$){date};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.08*(F.west)-0.08*(F.east)$){cumulative confirmed infections};
    \node[scale=0.8,anchor=east](P)at($(F.east|-F.north)+(-3,-0.5)$){prediction for 3/15};
  \end{tikzpicture}
  \vspace*{-10pt}
  \caption{\small
    Early dynamics of (USA) COVID-19 and model prediction.
    Dates are the time-stamps on the ECDC report, which captures the previous day's activity (e.g. the time stamp 1/21 is the infection on 1/20).\label{fig:model1}}
\end{figure}
We analyze daily confirmed COVID-19
from January 21 to March 14. Our model is \emph{time stamped}, hence
we can provably test it moving forward.
Our model predictions up to March 15 are in
Figure~\ref{fig:model1}. Red circles are cumulative confirmed
infections, the blue curve is our learned model and the blue circle is
our prediction for March~15,
665 new confirmed infections. Qualitatively the model captures the data.
The blue model curve is, in some sense, an optimal
fit to the data, with an \emph{asymptomatic}
infectious force if left unchecked
of 30\% new cases per day (doubling in about 2.6 days)
and a virulence of
\math{\gamma=0.14\%} (1 or 2 in a thousand conversions from mild infection
to serious). Not all serious cases are fatal.
Such early intelligence
has public
health significance:
stay calm, the virulence is not astonishingly high, but
the spread rate is high, hence one must
curtail that spread, or else a health-system can get overloaded.
Our contributions are
\begin{itemize}\itemsep-2pt\vspace*{-5pt}
\item A methodology for quickly and robustly machine learning
  (reverse engineering) simple
  epidemiological models given coarse aggregated infection counts.
\item Emphasizing the importance of early dynamics in learning the
  behavior of a pandemic.
\item Application of the methodology within the context of COVID-19
  to extract the pandemic parameters consistent with USA data. We
  also perform a cross-sectional analysis of the data across several
  countries.
\end{itemize}

  


\section{Model, Data and Analysis}

Our goal is a simple robust model.
The majority of disease models are
based on aggregation of individuals according to disease status,
such as SI, SIR, SIS, \cite{Kermack1927,Bailey1957,Anderson1992}.
We use a similar model by considering a mild infected state which can
transition to a serious state.
Early data allows us to make
simplifying assumptions. In the early phase, when public health
protocols have not kicked in, a confirmed infection is self-reported. That is,
\emph{you} decide to
get tested. Why? Because the condition became serious. This is
important. A confirmed case is a transition from
mild infection to serious. This is not true later when, for example,
public health
protocols may institute randomized testing. At
time \math{t} let there be \math{C(t)} confirmed cases and correspondingly
\math{M(t)} mild unreported asymptomatic infections. The new confirmed cases
at time \math{t} correspond to mild infections at some earlier time
\math{t-k} which have now transitioned to serious and hence
got self-reported.
Let us suppose that a fraction \math{\gamma} of those mild
cases transitioned to serious,
\mandc{C(t)=C(t-1)+\gamma M(t-k).}
Another
advantage of early dynamics is that we may approximate the growth from each
infection as independent and exponential, according to the infectious force
of the disease. So,
\mandc{M(t)=\beta M(t-1)-\gamma M(t-k)-(1-\gamma)M(t-k-r)+\alpha C(t-1).}
Here, the second term is the loss of mild cases that transitioned to
serious, the third term is the remaining 
cases that don't transition to serious
recovering at some later time \math{r}
  and the fourth term accounts for
new infections from
confirmed cases. We will further simplify and assume that confirmed cases
are fully quarantined and so \math{\alpha=0} and recovery to a non-infectious
state occurs
late enough to not factor into early dynamics. Our simplified model is:
\mldc{
  \begin{array}{rcl@{\hspace*{0.5in}}l}
  S(t)&=&S(t-1)+\gamma M(t-k)& S(t)=S(1)\text{ for } 1\le t<k\\
  M(t)&=&\beta M(t-1)-\gamma M(t-k)& M(1)=M_0.
  \end{array}
}
We set \math{t=1} at the first confirmed infection
(Jan 21 in USA). There are four parameters.
\myslimfbox[fillLightgray]{0.95\textwidth}{
\mandc{\arraycolsep2pt
  \begin{array}{rl}
    \beta,&\text{the asymptomatic
      infectious force parameter governing the exponential
      spreading}\\
    \gamma,&\text{the virulence, the fraction of mild cases that become
      serious some time later}\\
    k,&\text{the lag time for mild asymptomatic infection to become serious
      (incubation time)}\\
    M_0,& \text{The number of unconfirmed mild infections at the begining}
  \end{array}
}
}
We assess the quality of
the parameters \math{\beta,\gamma,k,M_0} by how well they
reproduce the
observed dynamics in Figure~\ref{fig:model1}, using an error-measure, see
for example \cite{malik173}.
We used a combination of
root-mean-squared-error  and root-mean-squared-percentage-error
between observed
dynamics and model predictions. The model parameters which optimally
fit the data are
\mldc{
  \beta^*=1.30\qquad\qquad
  \gamma^*=0.0014 \qquad\qquad
  k^*=10\text{ days}      \qquad\qquad
  M_0^*=4\label{eq:param-pot}
}
The asymptomatic infectious force, \math{\beta}, is very high, and corresponds
to a doubling time of 2.6 days. On the other hand, the
virulence at 0.14\% is small, comparable to a standard flu.
That is promising.
The incubation period of 10 days seems in line with physician
observations. The data analysis predicts that when
the first confirmed case appeared, there were 4 other infections in the USA.
The parameters \math{\beta^*, \gamma^*} and \math{M_0^*} are new knowledge,
gained with relative ease by calibrating a simple robust
model to the early dynamics. But, these optimal parameters are not the whole
story, when it comes to prediction.


Let us walk through the process of
obtaining the optimal parameters \math{(\beta^*,\gamma^*,k^*,M_0^*)}.
First we determined the incubation period
\math{k} and the number  of initial unseen mild infections \math{M_0}.
We exhaustively searched over \math{(k,M_0)} and for each
pair of values, we used gradient descent with 4 million iterations
to identify the optimal
\math{\beta} and \math{\gamma} for  that specific \math{k,M_0}.
We show the quality of fit
for various \math{(k,M_0)} in Figure~\ref{fig:model2}(a).
The deep-blue region contains essentially equivalent models within
0.5\% of the optimal fit, our (user defined) error tolerance.
The deep-blue region shows the extent to which the
model is ill-identified by the data. Indeed, all these deep-blue
models equally
fit the data which results in a range of predictions. For robustness, we
pick the white square in the middle of the deep-blue region, but note here that it
is only one of the models which are consistent
with the data. In making predictions, we
should consider all equivalent models to get a range for the predictions that
are all equally consistent with the data.
Similarly, in Figure~\ref{fig:model2}(b), we fix
\math{k^*} and \math{M_0^*} to their optimal robust values
and show the uncertainty with respect to
\math{\beta} and \math{\gamma} (the deep-blue region). Again, we pick the white square
in the middle of the deep-blue region of equivalent
models with respect to the data. Hence we arrive at our optimal
parameters in Equation \r{eq:param-pot}.



\begin{figure}[t]
  {\tabcolsep0pt
  \begin{tabular}{c@{\hspace*{0.025\textwidth}}c}
  \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics*[width=0.45\textwidth,trim={4.85cm 8cm 4.35cm 7.5cm},clip]{Fig2}};
    \foreach\x/\z[count=\i]in{{1}/0.98,{20}/0.02}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }
    \foreach\y/\z[count=\i]in{{1}/0.97,{20}/0.03}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
    }
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.04*(F.south)-0.04*(F.north)$){\math{M_0}, initial mild infections};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.03*(F.west)-0.03*(F.east)$){\math{k}, incubation period (days)};
  \end{tikzpicture}
  &
   \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics*[width=0.45\textwidth,trim={4.85cm 8cm 4.35cm 7.5cm},clip]{Fig3}};
    \foreach\x/\z[count=\i]in{{-0.46}/0.98,{1.14}/0.02}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }
    \foreach\y/\z[count=\i]in{{-18}/0.97,{18}/0.03}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
    }
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.04*(F.south)-0.04*(F.north)$){\math{1400\beta+35\gamma}};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.03*(F.west)-0.03*(F.east)$){\math{1400\beta-35\gamma}};
   \end{tikzpicture}
   \\
   (a)&(b)
  \end{tabular}
  }
  \vspace*{-8pt}
  \caption{\small Uncertainty in model estimation. (a) Optimal fit-error over
    for different choices of incubation period and
    initial infections. Blue is better fit, red is worse fit. The deep-blue
    region corresponds to comparable models, within 0.5\% of the
    optimal fit.
    The white square is the model chosen, \math{(k^*,M_0^*)=(10,4)}
    which has optimal fit and also is
    ``robust'' being in the middle of the deep-blue regions.
    (b) Model fit for the chosen \math{k^*} and \math{M_0^*}.
    Again, blue is a better fit and the deep-blue region is an equivalence
    class of optimal models. We choose the ``robust'' model
    corresponding to the
    white square in the middle of the deep-blue region,
    \math{(\beta^*,\gamma^*)=(1.30,0.0014)}
    The deep-blue regions represent uncertainty.\label{fig:model2}}
\end{figure}

\subsection{Cross-Sectional Study Across Countries}
In the supplementary material we give a cross-sectional study across
countries. The different countries have different
cultures, social networks, mobility, demographics, as well as different
times at which the first infection was reported (the ``delay'').
We show the resulting parameters reverse-engineered per country
in Table~\ref{tab:intro:country-fits}.
\begin{table}[!ht]  
\centering
{  \tabcolsep5pt
  \begin{tabular}{l||lc|lc|lc|lc}
    Country&\math{\beta}&\math{[{\min},{\max}]}&\math{\gamma}&\math{[{\min},{\max}]}&\math{k}&\math{[{\min},{\max}]}&\math{M_0}&\math{[{\min},{\max}]}\\\hline
Australia&1.143&[1.137,1.18]&0.0047&[0.0024,0.046]&2&[1,3]&10&[1,18]\\
Austria&1.411&[1.389,2.261]&0.045&[0.022,0.89]&1&[1,1]&20&[1,40]\\
Canada&1.182&[1.176,1.191]&0.0014&[0.00025,0.0099]&3&[1,3]&10&[1,40]\\
China&1.312&[1.297,1.332]&5.18&[3.75,8.26]&15&[14,16]&6&[5,9]\\
France&1.297&[1.293,1.301]&0.05&[0.0128,0.449]&19&[18,20]&7&[1,36]\\
Germany&1.289&[1.287,1.295]&0.011&[0.0039,0.044]&8&[1,8]&4&[1,10]\\
Iran&1.596&[1.563,1.709]&0.78&[0.71,0.79]&4&[3,4]&30&[29,40]\\
Ireland&1.401&[1.372,1.79]&0.083&[0.042,0.62]&2&[2,2]&20&[2,40]\\
Italy&1.242&[1.237,1.255]&3.88&[3.11,5.37]&19&[18,19]&6&[4,8]\\
Netherlands&1.387&[1.372,2.28]&0.34&[0.29,1.314]&4&[2,4]&35&[2,40]\\
Norway&1.461&[1.379,2.935]&0.164&[0.082,1.64]&1&[1,3]&20&[1,40]\\
Poland&1.476&[1.422,3.542]&0.109&[0.054,2.17]&1&[1,1]&20&[1,40]\\
Portugal&1.4&[1.356,3.077]&0.0886&[0.044,1.77]&1&[1,1]&20&[1,40]\\
South Africa&1.563&[1.513,2.65]&0.057&[0.031,1.15]&1&[1,2]&20&[1,37]\\
South Korea&1.238&[1.231,1.289]&0.98&[0.76,4.65]&20&[14,20]&7&[1,9]\\
Spain&1.411&[1.405,1.418]&0.127&[0.016,0.63]&20&[20,20]&5&[1,40]\\
Sweden&1.356&[1.343,1.372]&0.064&[0.0068,0.27]&19&[19,20]&3&[1,40]\\
Switzerland&1.527&[1.448,2.121]&0.4&[0.267,1.078]&3&[2,3]&12&[2,21]\\
UK&1.252&[1.248,1.257]&0.68&[0.412,0.878]&19&[17,20]&1&[1,1]\\
USA&1.306&[1.303,1.309]&0.0014&[0.0006,0.009]&10&[3,12]&4&[1,7]
\end{tabular}
}
\caption{Fit parameters for 20 countries.\label{tab:intro:country-fits}}
\end{table}
We primarily focus on 
the infectious force \math{\beta}, which has significant variability,
and we study how \math{\beta} statistically depends on a number of
country-specific parameters factors (see the supplementary material for
details). We find:
\begin{itemize}\itemsep-3pt\vspace*{-5pt}
\item
  The larger the delay, the larger is \math{\beta}. The more that has been
  witnessed, the faster the spread. That seems unusual, but
  is strongly indicated by the data.
\item Population density at the infection site has a strong
  positive effect but the country's population density does not.
\item
  There is faster spread in countries with more people under the
  poverty level defined as the percentage of people
  living on less than \$5.50 per day.
\item
  Median age has a strong effect. Spread is faster in younger populations.
  The youth are more mobile and perhaps also more carefree.
\item Wealth and per-capita income have a slight negative effect.
  Spread is slower in richer countries, perhaps due to some combination of
  more risk-aversion, higher levels of education and less
  reliance on public transportation. Whatever the cause, it does have an
  impact, but relatively smaller than the other effects.
  \vspace*{-5pt}
\end{itemize}

\section{Predictions and Discussion}

As mentioned in the previous section, to get honest estimates, we must
consider all models which are equally consistent with the data, indicated
by the deep-blue regions in Figure~\ref{fig:model2}.
We arrive at the following
ranges for our estimates, based on a 0.5\% error tolerance.
\mandc{\arraycolsep6pt\renewcommand{\arraystretch}{1.3}
  \begin{array}{ccccc}
    \beta (\beta^*=1.30)&\gamma (\gamma^*=0.14\%)&k (k^*=10\text{ days})&M_0 (M_0^*=4)&\text{Asymptomatic on 03/14}\\\hline
         [1.3,1.31]&[0.03\%,1.2\%]&[1\text{ day},13\text{ days}]&[1,12]&[1.3\text{ million},16\text{ million}]
  \end{array}
}
Asymptomatic
infectionis strong, around 30\%, however it is
not that virulent, converting at most 1.2\% of mild infections to serious.
There is significant uncertainty in the lag, from 1 up to
13 days, and there could have been up to 12 unknown initial infections
when the first case was confirmed. As of March 14, the model suggests
on the order of a million unknown infections.

We now come to predictions beyond
March 14, see Table~\ref{table:predictS} and Figure~\ref{fig:model3}. 
Data beyond March 14 was not used to calibrate the model.
You may complain about
the large uncertainty-range for each prediction.
Unfortunately, that is what the data tells
us. There is uncertainty, it's a fact of life. There are many
models equally consistent with the data,
resulting in a range of predictions. The model says that if the pandemic
is left to its business unchecked, we should expect a total of
about 29 thousand new
confirmed infections by March 24, and the range is from 28 to 125 thousand.
\begin{table}[t]
\small
  \centering
{\tabcolsep8pt\renewcommand{\arraystretch}{1.2}
  \begin{tabular}{r|cl|c}
    &\multicolumn{3}{c}{New Infections}\\
    Date&Model Prediction&\multicolumn{1}{l}{Range}&Observed\\\hline
    March 15, 2020&665&[657,2861]&\blue{\bf 777}\\
    March 16, 2020&866&[856,3732]&\red{\bf 823}\\
    March 17, 2020&1130&[1114,4867]&\red{\bf 887}\\
    March 18, 2020&1475&[1450,6348]&\blue{\bf 1766}\\
    March 19, 2020&1924&[1888,8280]&\blue{\bf 2988}\\
    March 20, 2020&2510&[2459,10800]&\blue{\bf 4835}\\
    March 21, 2020&3275&[3201,14088]&\blue{\bf 5374}\\
    March 22, 2020&4272&[4168,18375]&\blue{\bf 7123}\\
    March 23, 2020&5574&[5427,23968]&\blue{\bf 8459}\\
    March 24, 2020&7271&[7067,31263]&\blue{\bf 11236}\\
    March 25, 2020&9487&[9201,40789]&\red{\bf 8789}\\
    March 26, 2020&12376&[11980,53216]&\blue{\bf 13693}\\
    March 27, 2020&16146&[15198,69430]&\blue{\bf 16797}\\
    March 28, 2020&21065&[20309,90585]&\red{\bf 18695}\\
    March 29, 2020&27482&[26443,118180]&\red{\bf 19979}\\
    March 30, 2020&35854&[34430,154190]&\red{\bf 18360}
\end{tabular}}
\caption{Predictions of new infections by the learned  model and a range given by the space of models equally consistent with the data. March 15 and 16 data
  arrived at the time of writing and March 17 onward arrived after the time of
  writing. Blue means in the range and red means outside the range.
  Note that the new infections (a change in cumulative infections)
  is less stable than the cumulative infection predictions, which are
  shown in Figure~\ref{fig:model3}.
  \label{table:predictS}}
\end{table}

We can learn a lot from the early dynamics of COVID-19. It's infectious
force, virulence, incubation period, unseen infections and predictions of
new confirmed cases. All this, albeit within error tolerances, from a
simple model and little data. And, the information is useful for
planning and health-system preparedness. A side benefit of the predictions in
Table~\ref{table:predictS}, if the model is to be trusted, is as a benchmark 
against which to evaluate public health interventions. If moving forward,
observed new infections are low compared to the data in
Table~\ref{table:predictS}, it means the
interventions are working by most likely
reducing \math{\beta}.
The US instuted broad and aggressive social distancing protocols starting on
or before March 12. If our ``lag'' \math{k=10} is accurate, and the social
distancing protocols have
been effective at reducing \math{\beta}, the observed new infections
should drop below the predictions starting on or before March 22.
Without such a target to compare with, it would
be hard to evaluate intervention protocols.

Our approach is simple, general
and works with coarse, aggregated  data.
We end with some
limitations. First, the independent evolution of infection sites only applies
to early dynamics.  Hence,
when the model infections increase beyond some point, and
the pandemic begins to saturate the population,
a more sophisticated network model that
captures the dependence between infection sites
would be
needed~\cite{Balcan2009,Hill2010,Salathe2010,Keeling2005,Chinazzi2020}.
While we did present an optimal model, it should be taken with
a grain of salt because many models are nearly equivalent, resulting in 
prediction uncertainty. The model and the
interpretation of its parameters will change once public health
protocols kick in. The model may have to be re-calibrated
(for example if \math{\beta} decreases) and the parameters may have to
be reinterpreted (for example \math{\gamma} is a virulence only in the
self-reporting setting, not for random testing).
It is also possible to build a more general model with an early phase
\math{\beta_1} and a latter phase \math{\beta_2}
(after social distancing).
Lastly, the model was learned
on USA data. The learned model parameters may not be
appropriate for another society. The virulence could be globally
invariant, but it could also depend on genetic and demographic factors
like age, as well as what ``serious'' means for the culture - that is when
do you get yourself checked. In a high-strung society, you expect
high virulence since the threshold for serious is lower. One certainly expects 
the infectious force to depend on the underlying social network and
interaction patterns between people, which can vary drastically from one
society to another and depending on interventions.
Hence, one should
calibrate the model to country specific data to gain more useful insights.

\paragraph{Discussion.}
Early dynamics allows us to learn useful properties of the pandemic.
Later dynamics may be contaminated by human intervention,
which renders the data
not as useful without a more general model. Are our parameters
correct?
We are in a unique position to \emph{test} our predictions because our
model was \emph{time-stamped} as  version 1 of the
preprint~\cite{malik233}. The model has provably not changed,
and we just added in new test data as it arrives (Figure~\ref{fig:model3}).
The model predictions in Figure~\ref{fig:model3}
are in no way  forward looking, data snooped or overfitted. 
%Social distancing is a powerful tool against a
%pandemic as the graphic in Figure~\ref{fig:model3} shows.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[>=latex,line width=1pt]
    \node[inner sep=0pt](F)at(0,0){\includegraphics[width=0.6\textwidth,trim={1cm 6.7cm 1.35cm 6.9cm},clip]{Fig4}};
    \coordinate(TL)at(F.west|-F.north);
    \coordinate(BL)at(F.west|-F.south);
    \coordinate(TR)at(F.east|-F.north);
    \coordinate(BR)at(F.east|-F.south);    
    \def\Tbeg{46}
    \def\Tmid{53}
    \def\Tlock{61}
    \def\Tend{72.5}
    \def\Tfinal{70}
    \def\datefinal{3/30}
    \def\ymin{1}
    \def\ymax{2950.4}
    \def\pow{0.65}

    \foreach\y/\x[count=\i]in{46/{3/7},\Tmid/{3/13},54.75/{3/14},\Tlock/{3/21},\Tfinal/{\datefinal}}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y-\Tbeg+0.5)/(\Tend-\Tbeg+1)}
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.65,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(BL)+\z*\lambar*(TL)+\zbar*\lam*(BR)+\zbar*\lambar*(TR)$){\x};
    }
    \foreach\y/\ty[count=\i]in{50/5,100/10,200/20,500/50,1000/100,2000/200}{
      \pgfmathsetmacro\lam{0.97};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(100^\pow*\y^(\pow)-\ymin+6)/(\ymax-\ymin+12)}
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.7,anchor=east](x\i)at($\z*\lam*(BL)+\z*\lambar*(BR)+\zbar*\lam*(TL)+\zbar*\lambar*(TR)$){\ty};
    }
    \pgfmathsetmacro\xlam{(\Tlock.3-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlock)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\xlam{(\Tlock.3+10-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlocklag)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(100^(\pow)*1150^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylock)at($\ylambar*(BL)+\ylam*(TL)$);
    \pgfmathsetmacro\xlam{(\Tmid.3-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlast)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(100^(\pow)*320^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylast)at($\ylambar*(BL)+\ylam*(TL)$);
    \pgfmathsetmacro\xlam{(\Tmid.3+10.25-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlag)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(4000^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylag)at($\ylambar*(BL)+\ylam*(TL)$);
    \path
    ($(xlast|-ylast)$)edge[->]node[above=6pt,scale=0.8,inner sep=0pt,pos=0.05,anchor=west]{social distancing}node[below=6pt,scale=0.8,inner sep=0pt,pos=0.05,anchor=west]{lag, \math{k=10}}(xlag|-ylast)
    ($(xlock|-ylock)$)edge[->]node[above=6pt,scale=0.8,inner sep=0pt,pos=0.05,anchor=west]{lockdown}node[below=6pt,scale=0.8,inner sep=0pt,pos=0.05,anchor=west]{lag, \math{k=10}}(xlocklag|-ylock)
    ;    
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.06*(F.south)-0.06*(F.north)$){date};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.08*(F.west)-0.08*(F.east)$){cumulative confirmed infections (\math{\times 1000})};
    \node(C)at($(F)+(-3.5,+1)$){\color{fillgray}\textsc{\begin{tabular}{c}Training\\the\\Model\end{tabular}}};
  \end{tikzpicture}
  \vspace*{-10pt}
  \caption{\small
    Testing model predictions (the blue envelope indicates the predicted
    range).
    The gray region is data used to train the model.
    A falloff of observed
    infections away from predicted infections indicates that 
    social distancing is working, and we predict a lag for that of 10 days.
    As can be seen, visually, there are two ``kinks'' in the curve at about
    the times predicted by the lag \math{k=10}. The figure also illustrates
    the need to focus on early data to learn about the pandemic, as the
    later data now contaminated by public health protocols whose
    effects are hard to quantify.
    \label{fig:model3}}
\end{figure}
Training used only
data before 03/14.
The model
is holding up.

\emph{The Lag, \math{k}, and Public Policy.}
The lag \math{k} is
important for public policy. Our lag, \math{k=10}, says 
the confirmed infections should fall away from the predictions on about
03/22,
because  aggressive social distancing
began on around 03/12. We actually observe a phase change/fall off
on or around
03/24.
The lag is important due to how public policy can be
driven by human psychology as opposed to quantitative models.
March 20 saw a 40\% increase in new infections compared to the previous day.
This led to a significant heightening of vigilance and
calls for ``shelter in place''  protocols.
But, by March 20, we still do not know the effectiveness of social distancing
protocols from March 12th have been. Hence, such calls to vigilance
can be premature.
More importantly, suppose strict shelter in place protocols are enacted
on March 21 and
infections fall the next day. The Human tendency is to associate
the improvement to the March 21 strict protocols.
But, if the model is correct, the March 21 protocols have 
nothing to do with the improvement \emph{in observed
  infections} on March 22.
Such lags are present in traditional machine learning, for example
the delayed reward in reinforcement learning settings. Credit assignment
to prior actions in the face of delayed reward is a notoriously difficult
task, and this remains so with humans in the loop. Knowledge of the lag
helps to assign credit appropriately to prior actions, and the
public health setting is no exception.



%The observed lag of
%\math{k=????} is well inside the deep-blue
%region in Figure~\ref{fig:model2}.

\paragraph{Acknowledgments.}
We thank Abhijit Patel, Sibel Adali and Zainab Magdon-Ismail for
provoking discussions on this topic.




==> intro-2.tex <==
\section{Introduction}
\label{section:intro}

As of March 1 2020, there was still much public debate about properties
of the COVID-19 pandemic
(see the CNN article, \cite{CNN2020}). For example, is
asymptomatic spread of COVID-19 a major driver of the pandemic?
There was no clear unimodal view, and this highlights the
need for robust tools to generate actionable quantitative
intelligence on the nature
of a pandemic from \emph{early} and minimal data.
One approach is scenario analysis.
Recently, \cite{Chinazzi2020} used
the Global Epidemic and Mobility Model (GLEAM)
to perform infection scenario analyses on China COVID-19
data, using
a networked meta-population model based on transportation hubs.
A similar model for the US was reported in \cite{TIME2020} where their
web-app predicts from 150,000 to 1.4 million infected cases by April 30,
depending on the intervention level.
Such scenario analysis requires user input such as infection
sites and properties of the contagion. However,
a majority of infection sites may be hidden, especially if asymptomatic
transmission is significant. Further, the contagion parameters are
\emph{unknown} and 
must be deduced, perhaps using domain expertise.

Data driven approaches are powerful. A long range regression analysis of
COVID-19 out to 2025 on US data using immunological,
epidemiological and seasonal
effects is given in \cite{Kissler2020},
which predicts  recurrent outbreaks.
We also follow a pure data-driven machine learning
approach to understand early dynamics of COVID-19 on the first
54 days of US confirmed infection reports (downloadable from
the European Center For Disease Control).
We address the challenge of real-time data-intelligence from early data.
Our data-approach
is simple, requires minimal data or human input and generates
actionable insights.
For example, is asymptomatic spread significant?
Our data-driven analysis says yes, emphatically, and we can get quantitative
estimates
of the number of asymptomatic infections.

Early data
is both a curse and a blessing.
The curse is that ``early'' implies not
much information, so quantitative models must be simple and robust
to be identifiable from the data.
The blessing is that early data is
a peek at the pandemic as it roams free,
unchecked by public health protocols, for
to learn the true intentions of the lion, you must follow the
beast on the savanna, not in the zoo.
As we will see, much can be learned from early data and
these insights early in the game,
can be crucial to public health governance.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[>=latex,line width=1pt]
    \node[inner sep=0pt](F)at(0,0){\includegraphics[width=0.8\textwidth,trim={1cm 6.7cm 1.35cm 6.9cm},clip]{Fig4}};
    \coordinate(TL)at(F.west|-F.north);
    \coordinate(BL)at(F.west|-F.south);
    \coordinate(TR)at(F.east|-F.north);
    \coordinate(BR)at(F.east|-F.south);    
    \def\Tbeg{46}
    \def\Tmid{53}
    \def\Tlock{61}
    \def\Tend{74.5}
    \def\Tfinal{73}
    \def\datefinal{4/2}
    \def\ymin{1}
    \def\ymax{3527.8}
    \def\pow{0.65}

    \foreach\y/\x[count=\i]in{46/{3/7},\Tmid/{3/13},54.75/{3/14},\Tlock/{3/21},70/{3/30},\Tfinal/{\datefinal}}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y-\Tbeg+0.5)/(\Tend-\Tbeg+1)}
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(BL)+\z*\lambar*(TL)+\zbar*\lam*(BR)+\zbar*\lambar*(TR)$){\x};
    }
    \foreach\y/\ty[count=\i]in{50/5,100/10,200/20,500/50,1000/100,2000/200}{
      \pgfmathsetmacro\lam{0.97};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(100^\pow*\y^(\pow)-\ymin+6)/(\ymax-\ymin+12)}
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,anchor=east](x\i)at($\z*\lam*(BL)+\z*\lambar*(BR)+\zbar*\lam*(TL)+\zbar*\lambar*(TR)$){\ty};
    }
    \pgfmathsetmacro\xlam{(\Tlock.4-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlock)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\xlam{(\Tlock.4+10-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlocklag)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(100^(\pow)*1150^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylock)at($\ylambar*(BL)+\ylam*(TL)$);
    \pgfmathsetmacro\xlam{(\Tmid.4-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlast)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(100^(\pow)*320^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylast)at($\ylambar*(BL)+\ylam*(TL)$);
    \pgfmathsetmacro\xlam{(\Tmid.4+10.25-\Tbeg+0.4)/(\Tend-\Tbeg+0.8)};
    \pgfmathsetmacro\xlambar{1-\xlam};
    \coordinate(xlag)at($\xlambar*(BL)+\xlam*(BR)$);
    \pgfmathsetmacro\ylam{(4000^(\pow)-\ymin+6)/(\ymax-\ymin+12)};
    \pgfmathsetmacro\ylambar{1-\ylam};
    \coordinate(ylag)at($\ylambar*(BL)+\ylam*(TL)$);
    \path
    ($(xlast|-ylast)$)edge[->]node[above=6pt,scale=0.9,inner sep=0pt,pos=0.05,anchor=west]{social distancing}node[below=6pt,scale=0.9,inner sep=0pt,pos=0.05,anchor=west]{lag, \math{k=10}}(xlag|-ylast)
    ($(xlock|-ylock)$)edge[->]node[above=6pt,scale=0.9,inner sep=0pt,pos=0.05,anchor=west]{lockdown}node[below=6pt,scale=0.9,inner sep=0pt,pos=0.05,anchor=west]{lag, \math{k=10}}(xlocklag|-ylock)
    ;    
    \node[scale=1,inner sep=0pt](xlabel)at($1.04*(F.south)-0.04*(F.north)$){date};
    \node[scale=1,rotate=90,inner sep=0pt](ylabel)at($1.04*(F.west)-0.04*(F.east)$){cumulative confirmed infections (\math{\times 1000})};
    \node(C)at($(F)+(-4.5,+1)$){\color{fillgray}\textsc{\begin{tabular}{c}Training\\the\\Model\end{tabular}}};
  \end{tikzpicture}
  \vspace*{-10pt}
  \caption{\small
    Testing model predictions (the blue envelope indicates the predicted
    range).
    The gray region is data used to train the model.
    A falloff of observed
    infections away from predicted infections indicates that 
    social distancing is working, and we predict a lag for that of 10 days.
    As can be seen, visually, there are two ``kinks'' in the curve at about
    the times predicted by the lag \math{k=10}. The figure also illustrates
    the need to focus on early data to learn about the pandemic, as
    later data is ``contaminated'' by public health protocols whose
    effects are hard to quantify. (Note: Dates are the time-stamps on the ECDC report \citep{ECDC2020}, which captures the previous day's activity)
    \label{fig:model3}}
\end{figure}

We analyzed daily confirmed COVID-19 cases
from January 21 to March 14, the training or model calibration phase, the
gray region in Figure~\ref{fig:model3}. A more detailed plot of the model fit to
the training data is in Figure~\ref{fig:model1}.
Qualitatively we see that the model captures the data, and it does so
by setting
four parameters:
\myslimfbox[fillLightgray]{0.95\textwidth}{
\math{\arraycolsep2pt
  \begin{array}{rl}
    \beta,&\text{the {\bf asymptomatic}
      infectious force parameter governing the exponential
      spread}\\
    \gamma,&\text{the virulence, the fraction of mild cases that become
      serious some time later}\\
    k,&\text{the lag time for mild asymptomatic infection to become serious
      (an incubation time)}\\
    M_0,& \text{The number of unconfirmed mild asymptomatic
      infections at the begining}
  \end{array}
}
}
By calibrating the model to the training data, we obtain the following
information.
\mldc{\arraycolsep8pt\renewcommand{\arraystretch}{1.2}
  \begin{array}{l|ll}
    \text{parameter}&\text{model}&\text{range}\\\hline
    \text{asymptomatic
    infectious force }\beta&\beta^*=1.30&[1.3,1.31]
\\
\text{virulence }\gamma&\gamma^*=0.14\%&[0.03\%,1.2\%]
\\
\text{lag }k&k^*=10\text{ days}&[1\text{ day},13\text{ days}]
\\
\text{initial infections }M_0&M_0^*=4&[1,12]
\\
\text{asymptomatic on 03/14 }&5.3\text{ million}&[1.3\text{ million},26\text{ million}]
\end{array}
  \label{eq:model1}
}
The \emph{asymptomatic}
infectious force if left unchecked is
30\% new cases per day (doubling in about 2.6 days)
and the virulence is
\math{\gamma=0.14\%} (1 or 2 in a thousand conversions from mild infection
to serious). Not all serious cases are fatal.
The model output about 5.3 million asymptomatic cases as of 03/14 and a range
from 1 to 26 million, a surprisingly high number.
Such quantitative early intelligence
has significance for public
health protocols.

Beyond 03/14 in Figure~\ref{fig:model3} are the model
predictions (blue line and shaded blue region) and the red circles are
the observed infection counts. First, do we know that the model predictions
are honest, in that the red circles were in no way used to generate the
predictions. Yes! We are in a unique position to test the model because
the model is \emph{time stamped} as as  version 1 of the
preprint~\cite{malik233}.
The model has provably not changed since 03/14,
and we just added new test data as it arrived.
Hence, the model predictions in Figure~\ref{fig:model3}
are in no way  forward looking, data snooped or overfitted.
Moving forward, we observe that the model and observed counts agree,
modulo two ``kinks'' around 03/24 and 03/30, when the observed
infections start falling away from the model. To understand the cause, the
lag is important. Aggressive social distancing was implemented on about
03/13 and lockdowns around 03/21. A lag of \math{k=10} means the effects of
these protocols will become apparent around 03/23 and 03/31 respectively.

The methods are general and can be applied to different cohorts. In
Section~\ref{} we do a cross-sectional country-based study of the
pandemic properties, and in Section~\ref{} we study cohorts based on
virus strain. A summary of our contributions are
\begin{itemize}\itemsep-2pt\vspace*{-5pt}
\item A methodology for quickly and robustly machine learning
  (reverse engineering) simple
  epidemiological models given coarse aggregated infection counts.
\item Emphasizing the importance of early dynamics in learning the
  behavior of a pandemic.
\item Application of the methodology within the context of COVID-19
  to extract the pandemic parameters consistent with USA data.
\item Cross-sectional analysis of the pandemic dynamics across several
  countries.
\item Cross-sectional analysis of the pandemic dynamics based on virus
  strains.
\end{itemize}




\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics[width=0.8\textwidth,trim={1cm 6.7cm 1.35cm 6.9cm},clip]{Fig1}};
    \foreach\y/\x[count=\i]in{1/{1/21},10/{2/1},20/{2/10},30/{2/20},40/{3/1},50/{3/10},54/{3/14}}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y-1+1.5)/(55-1+3)}%xmin=1,xmax=55
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.75,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }

    \foreach\y[count=\i]in{500,1000,1500,2000,2180}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\z{1-(\y^(0.75)+1+4)/(330.05+1+8)}%ymin=-1,ymax=330.05
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.65,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
      }
    
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.06*(F.south)-0.06*(F.north)$){date};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.08*(F.west)-0.08*(F.east)$){cumulative confirmed infections};    
  \end{tikzpicture}
  \vspace*{-10pt}
  \caption{\small
    Model calibration to the early dynamics (first 54 infection counts)
    of (USA) COVID-19.
    Dates are the time-stamps on the ECDC report, which captures the previous day's activity (e.g. the time stamp 1/21 is the infection on 1/20).\label{fig:model1}}
\end{figure}
  
\section{Model and Method}

Our goal is a simple robust model.
The majority of disease models are
based on aggregation of individuals according to disease status,
such as SI, SIR, SIS, \cite{Kermack1927,Bailey1957,Anderson1992}.
We use a similar model by considering a mild infected state which can
transition to a serious state.
Early data allows us to make
simplifying assumptions. In the early phase, when public health
protocols have not kicked in, a confirmed infection is self-reported. That is,
\emph{you} decide to
get tested. Why? Because the condition became serious. This is
important. A confirmed case is a transition from
mild infection to serious. This is not true later when, for example,
public health
protocols may institute randomized testing. At
time \math{t} let there be \math{C(t)} confirmed cases and correspondingly
\math{M(t)} mild unreported asymptomatic infections. The new confirmed cases
at time \math{t} correspond to mild infections at some earlier time
\math{t-k} which have now transitioned to serious and hence
got self-reported.
Let us suppose that a fraction \math{\gamma} of those mild
cases transitioned to serious,
\mandc{C(t)=C(t-1)+\gamma M(t-k).}
Another
advantage of early dynamics is that we may approximate the growth from each
infection as independent and exponential, according to the infectious force
of the disease. So,
\mandc{M(t)=\beta M(t-1)-\gamma M(t-k)-(1-\gamma)M(t-k-r)+\alpha C(t-1).}
Here, the second term is the loss of mild cases that transitioned to
serious, the third term is the remaining 
cases that don't transition to serious
recovering at some later time \math{r}
  and the fourth term accounts for
new infections from
confirmed cases. We will further simplify and assume that confirmed cases
are fully quarantined and so \math{\alpha=0} and recovery to a non-infectious
state occurs
late enough to not factor into early dynamics. Our simplified model is:
\mldc{
  \begin{array}{rcl@{\hspace*{0.5in}}l}
  S(t)&=&S(t-1)+\gamma M(t-k)& S(t)=S(1)\text{ for } 1\le t<k\\
  M(t)&=&\beta M(t-1)-\gamma M(t-k)& M(1)=M_0.
  \end{array}
}
We set \math{t=1} at the first confirmed infection
(Jan 21 in USA). 
We assess the quality of
the parameters \math{\beta,\gamma,k,M_0} by how well they
reproduce the
observed dynamics in Figure~\ref{fig:model1}, using an error-measure, see
for example \cite{malik173}.
We used a combination of
root-mean-squared-error  and root-mean-squared-percentage-error
between observed
dynamics and model predictions. The optimal fit to the training data is
shown in
Figure~\ref{fig:model1} and the model parameters which optimally
fit the data are
\mldc{
  \beta^*=1.30\qquad\qquad
  \gamma^*=0.0014 \qquad\qquad
  k^*=10\text{ days}      \qquad\qquad
  M_0^*=4\label{eq:param-pot}
}
The asymptomatic infectious force, \math{\beta}, is very high, and corresponds
to a doubling time of 2.6 days. On the other hand, the
virulence at 0.14\% seems comparable to a standard flu, though the virus
may be affecting certain demographics much more severely than a flu.
The incubation period of 10 days seems in line with physician
observations. The data analysis predicts that when
the first confirmed case appeared, there were 4 other infections in the USA.
The parameters \math{\beta^*, \gamma^*} and \math{M_0^*} are new knowledge,
gained with relative ease by calibrating a simple robust
model to the early dynamics. But, these optimal parameters are not the whole
story, especially when it comes to prediction.



\begin{figure}[t]
  {\tabcolsep0pt
  \begin{tabular}{c@{\hspace*{0.025\textwidth}}c}
  \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics*[width=0.45\textwidth,trim={4.85cm 8cm 4.35cm 7.5cm},clip]{Fig2}};
    \foreach\x/\z[count=\i]in{{1}/0.98,{20}/0.02}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }
    \foreach\y/\z[count=\i]in{{1}/0.97,{20}/0.03}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
    }
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.04*(F.south)-0.04*(F.north)$){\math{M_0}, initial mild infections};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.03*(F.west)-0.03*(F.east)$){\math{k}, incubation period (days)};
  \end{tikzpicture}
  &
   \begin{tikzpicture}
    \node[inner sep=0pt](F)at(0,0){\includegraphics*[width=0.45\textwidth,trim={4.85cm 8cm 4.35cm 7.5cm},clip]{Fig3}};
    \foreach\x/\z[count=\i]in{{-0.46}/0.98,{1.14}/0.02}{
      \pgfmathsetmacro\lam{1};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,inner sep=0pt,anchor=north](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.west|-F.north)+\zbar*\lam*(F.east|-F.south)+\zbar*\lambar*(F.east|-F.north)$){\x};
    }
    \foreach\y/\z[count=\i]in{{-18}/0.97,{18}/0.03}{
      \pgfmathsetmacro\lam{0.98};
      \pgfmathsetmacro\lambar{1-\lam};
      \pgfmathsetmacro\zbar{1-\z};
      \node[scale=0.8,anchor=east](x\i)at($\z*\lam*(F.west|-F.south)+\z*\lambar*(F.east|-F.south)+\zbar*\lam*(F.west|-F.north)+\zbar*\lambar*(F.east|-F.north)$){\y};
    }
    \node[scale=0.9,inner sep=0pt](xlabel)at($1.04*(F.south)-0.04*(F.north)$){\math{1400\beta+35\gamma}};
    \node[scale=0.9,rotate=90,inner sep=0pt](ylabel)at($1.03*(F.west)-0.03*(F.east)$){\math{1400\beta-35\gamma}};
   \end{tikzpicture}
   \\
   (a)&(b)
  \end{tabular}
  }
  \vspace*{-8pt}
  \caption{\small Uncertainty in model estimation. (a) Optimal fit-error over
    for different choices of incubation period and
    initial infections. Blue is better fit, red is worse fit. The deep-blue
    region corresponds to comparable models, within 0.5\% of the
    optimal fit.
    The white square is the model chosen, \math{(k^*,M_0^*)=(10,4)}
    which has optimal fit and also is
    ``robust'' being in the middle of the deep-blue regions.
    (b) Model fit for the chosen \math{k^*} and \math{M_0^*}.
    Again, blue is a better fit and the deep-blue region is an equivalence
    class of optimal models. We choose the ``robust'' model
    corresponding to the
    white square in the middle of the deep-blue region,
    \math{(\beta^*,\gamma^*)=(1.30,0.0014)}
    The deep-blue regions represent uncertainty.\label{fig:model2}}
\end{figure}
Let us walk through the process of
obtaining the optimal parameters \math{(\beta^*,\gamma^*,k^*,M_0^*)}.
First we determined the incubation period
\math{k} and the number  of initial unseen mild infections \math{M_0}.
We exhaustively searched over \math{(k,M_0)} and for each
pair of values, we used gradient descent with 4 million iterations
to identify the optimal
\math{\beta} and \math{\gamma} for  that specific \math{k,M_0}.
Some details on how to efficiently obtain these optimal \math{\beta,\gamma}
are given in the supplementary materials.
We show the quality of fit
for various \math{(k,M_0)} in Figure~\ref{fig:model2}(a).
The deep-blue region contains essentially equivalent models within
0.5\% of the optimal fit, our (user defined) error tolerance.
The deep-blue region shows the extent to which the
model is ill-identified by the data. Indeed, all these deep-blue
models equally
fit the data which results in a range of predictions. For robustness, we
pick the white square in the middle of the deep-blue region, but note here that it
is only one of the models which are consistent
with the data. In making predictions, we
should consider all equivalent models to get a range for the predictions that
are all equally consistent with the data.
Similarly, in Figure~\ref{fig:model2}(b), we fix
\math{k^*} and \math{M_0^*} to their optimal robust values
and show the uncertainty with respect to
\math{\beta} and \math{\gamma} (the deep-blue region). Again, we pick the white square
in the middle of the deep-blue region of equivalent
models with respect to the data. Hence we arrive at our optimal
parameters in Equation \r{eq:param-pot}. 
By considering all models which are equally consistent with the data, we
get the estimates toghether with the ranges in Equation~\ref{eq:model1}.

\section{Results}
As mentioned in the previous section, to get honest estimates, we must
consider all models which are equally consistent with the data, indicated
by the deep-blue regions in Figure~\ref{fig:model2}.

\subsection{COVID-19 in USA}
The model parameters are in Equation~\ref{eq:model1}, and the
prediction of new infections are in the table below. The cumulative
sum of the predicted infections is the
data plotted in Figure~\ref{fig:model3}.
\mandc{\text{\tabcolsep8pt\renewcommand{\arraystretch}{1.1}
  \begin{tabular}{r|cl|c}
    &\multicolumn{3}{c}{New Infections}\\
    Date&Model Prediction&\multicolumn{1}{l}{Range}&Observed\\\hline
    March 15, 2020&665&[657,2861]&\blue{\bf 777}\\
    March 16, 2020&866&[856,3732]&\red{\bf 823}\\
    March 17, 2020&1130&[1114,4867]&\red{\bf 887}\\
    March 18, 2020&1475&[1450,6348]&\blue{\bf 1766}\\
    March 19, 2020&1924&[1888,8280]&\blue{\bf 2988}\\
    March 20, 2020&2510&[2459,10800]&\blue{\bf 4835}\\
    March 21, 2020&3275&[3201,14088]&\blue{\bf 5374}\\
    March 22, 2020&4272&[4168,18375]&\blue{\bf 7123}\\
    March 23, 2020&5574&[5427,23968]&\blue{\bf 8459}\\
    March 24, 2020&7271&[7067,31263]&\blue{\bf 11236}\\
    March 25, 2020&9487&[9201,40789]&\red{\bf 8789}\\
    March 26, 2020&12376&[11980,53216]&\blue{\bf 13693}\\
    March 27, 2020&16146&[15198,69430]&\blue{\bf 16797}\\
    March 28, 2020&21065&[20309,90585]&\red{\bf 18695}\\
    March 29, 2020&27482&[26443,118180]&\red{\bf 19979}\\
    March 30, 2020&35854&[34430,154190]&\red{\bf 18360}\\
    March 31, 2020&46777&[44829,201170]&\red{\bf 21595}\\
    April 1, 2020&61026&[58369,262470]&\red{\bf 24998}\\
    April 2, 2020&79617&[75999,343440]&\red{\bf 27103}\\
\end{tabular}}}
The predictions are from the optimal model in \r{eq:model1}
and the ranges are obtained by using
the space of models equally consistent with the data. March 15 and 16 data
  arrived at the time of writing and March 17 onward arrived after the time of
  writing time-stamped version 1 \citep{malik233}.
  Blue means in the range and red means outside the range.
It may be frustrating that the uncertainty-range for each prediction is large.
Unfortunately, that is what the data tells
us. There are many
models equally consistent with the data,
resulting in a range of predictions. 


  \subsection{Cross-Sectional Study By Countries}
  
In the supplementary material we give details of our
cross-sectional study across
countries. The different countries have different
cultures, social networks, mobility, demographics, as well as different
times at which the first infection was reported (the ``delay'').
We calibrated independent models for each country and the
resulting model parameters are 
in Table~\ref{tab:intro:country-fits}.
\begin{table}[!t]  
\centering
{  \tabcolsep5pt
  \begin{tabular}{l||lc|lc|lc|lc}
    Country&\math{\beta}&\math{[{\min},{\max}]}&\math{\gamma}&\math{[{\min},{\max}]}&\math{k}&\math{[{\min},{\max}]}&\math{M_0}&\math{[{\min},{\max}]}\\\hline
Australia&1.143&[1.137,1.18]&0.0047&[0.0024,0.046]&2&[1,3]&10&[1,18]\\
Austria&1.411&[1.389,2.261]&0.045&[0.022,0.89]&1&[1,1]&20&[1,40]\\
Canada&1.182&[1.176,1.191]&0.0014&[0.00025,0.0099]&3&[1,3]&10&[1,40]\\
China&1.312&[1.297,1.332]&5.18&[3.75,8.26]&15&[14,16]&6&[5,9]\\
France&1.297&[1.293,1.301]&0.05&[0.0128,0.449]&19&[18,20]&7&[1,36]\\
Germany&1.289&[1.287,1.295]&0.011&[0.0039,0.044]&8&[1,8]&4&[1,10]\\
Iran&1.596&[1.563,1.709]&0.78&[0.71,0.79]&4&[3,4]&30&[29,40]\\
Ireland&1.401&[1.372,1.79]&0.083&[0.042,0.62]&2&[2,2]&20&[2,40]\\
Italy&1.242&[1.237,1.255]&3.88&[3.11,5.37]&19&[18,19]&6&[4,8]\\
Netherlands&1.387&[1.372,2.28]&0.34&[0.29,1.314]&4&[2,4]&35&[2,40]\\
Norway&1.461&[1.379,2.935]&0.164&[0.082,1.64]&1&[1,3]&20&[1,40]\\
Poland&1.476&[1.422,3.542]&0.109&[0.054,2.17]&1&[1,1]&20&[1,40]\\
Portugal&1.4&[1.356,3.077]&0.0886&[0.044,1.77]&1&[1,1]&20&[1,40]\\
South Africa&1.563&[1.513,2.65]&0.057&[0.031,1.15]&1&[1,2]&20&[1,37]\\
South Korea&1.238&[1.231,1.289]&0.98&[0.76,4.65]&20&[14,20]&7&[1,9]\\
Spain&1.411&[1.405,1.418]&0.127&[0.016,0.63]&20&[20,20]&5&[1,40]\\
Sweden&1.356&[1.343,1.372]&0.064&[0.0068,0.27]&19&[19,20]&3&[1,40]\\
Switzerland&1.527&[1.448,2.121]&0.4&[0.267,1.078]&3&[2,3]&12&[2,21]\\
UK&1.252&[1.248,1.257]&0.68&[0.412,0.878]&19&[17,20]&1&[1,1]\\
USA&1.306&[1.303,1.309]&0.0014&[0.0006,0.009]&10&[3,12]&4&[1,7]
\end{tabular}
}
\caption{Fit parameters for 20 countries.\label{tab:intro:country-fits}}
\end{table}

We primarily focused on 
the infectious force \math{\beta}, which has significant variability,
and we studied how \math{\beta} statistically depends on a number of
country-specific parameters factors. In the supplementary material, we
give details of the study and the quantitative results.  Qualitatively, we
find:
\begin{itemize}\itemsep-3pt\vspace*{-5pt}
\item
  The larger the delay in the virus reaching a country,
  the larger is \math{\beta}. The more that has been
  witnessed, the faster the spread. That seems unusual, but
  is strongly indicated by the data. We do not have a good explanation for
  this effect. It could be an artefact of testing procedures not being
  streamlined, so early adopters of the pandamic presenting as serious were
  just not being detected.
  
\item Population density at the infection site has a strong
  positive effect but the country's population density does not.
\item
  There is faster spread in countries with more people under the
  poverty level defined as the percentage of people
  living on less than \$5.50 per day.
\item
  Median age has a strong effect. Spread is faster in younger populations.
  The youth are more mobile and perhaps also more carefree.
\item Wealth and per-capita income have a slight negative effect.
  Spread is slower in richer countries, perhaps due to some combination of
  more risk-aversion, higher levels of education and less
  reliance on public transportation. Whatever the cause, it does have an
  impact, but relatively smaller than the other effects.
  \vspace*{-5pt}
\end{itemize}

\subsection{Cross-Sectional Study By Virus Strain}

\section{Conclusion}

Early dynamics allows us to learn useful properties of the pandemic.
Later dynamics may be contaminated by human intervention,
which renders the data
not as useful without a more general model.
We learned a lot from the early dynamics of COVID-19.
It's infectious
force, virulence, incubation period, unseen infections and predictions of
new confirmed cases. All this, albeit within error tolerances, from a
simple model and little data.
Asymptomatic
infection is strong, around 30\%,
not that virulent, converting at most 1.2\% of mild infections to serious.
There is significant uncertainty in the lag, from 1 up to
13 days, and we estimate 5.3 million asymptomatic infections as of 03/14, the
range being from 1 to 26 million.
Such information is useful for
planning and health-system preparedness.
Are our parameters
correct?
We were in a unique position to \emph{test} our predictions because our
model was \emph{time-stamped} as  version 1 of the
preprint~\cite{malik233}. 

A side benefit of model predictions, if the model is to be trusted, is as a benchmark 
against which to evaluate public health interventions. If moving forward,
observed new infections are low compared to the data in, it means the
interventions are working by most likely
reducing \math{\beta}. Starting on about March 25, the observed infections
starts falling off and we observe a flattening by March 28. 
The US instuted broad and aggressive social distancing protocols starting on
or before March 13 and even
stronger lockdown around March 21, which is consistent
with the data and the model's lag of \math{k=10}.
Without such quantitative targets to compare with, it would
be hard to evaluate intervention protocols.

Our approach is simple, general
and works with coarse, aggregated  data.
It has 
limitations.
\begin{itemize}\itemsep-2pt\vspace*{-5pt}
\item
  The independent evolution of infection sites only applies
to early dynamics.  Hence,
when the model infections increase beyond some point, and
the pandemic begins to saturate the population,
a more sophisticated network model that
captures the dependence between infection sites
would be
needed~\cite{Balcan2009,Hill2010,Salathe2010,Keeling2005,Chinazzi2020}.

\item
  While we did present an optimal model, it should be taken with
a grain of salt because many models are nearly equivalent, resulting in 
prediction uncertainty.

\item
  The model and the
interpretation of its parameters will change once public health
protocols kick in. The model may have to be re-calibrated
(for example if \math{\beta} decreases) and the parameters may have to
be reinterpreted (for example \math{\gamma} is a virulence only in the
self-reporting setting, not for random testing).
It is also possible to build a more general model with an early phase
\math{\beta_1} and a latter phase \math{\beta_2}
(after social distancing).
But, beware, for a more general sophisticated model looks
good \emph{a priori} until ti comes time to calibrate it to data, at which
point it becomes unidentifiable.

\item The model was learned
on USA data. The learned model parameters may not be
appropriate for another society. The virulence could be globally
invariant, but it could also depend on genetic and demographic factors
like age, as well as what ``serious'' means for the culture - that is when
do you get yourself checked. In a high-strung society, you expect
high virulence-parameter
since the threshold for serious is lower. One certainly expects 
the infectious force to depend on the underlying social network and
interaction patterns between people, which can vary drastically from one
society to another and depending on interventions.
Hence, one should
calibrate the model to country specific data to gain more useful insights.
\vspace*{-5pt}
\end{itemize}
\emph{The Lag, \math{k}, and Public Policy.}
The lag \math{k} is
important for public policy due to how public policy can be
driven by human psychology.
The Human tendency is to associate
any improvement in outcome to recent actions. However, if there is
a lag, one might prematurely reward those recent actions
instead of the earlier actions whose effects are actually being seen.
Such lags are present in traditional machine learning, for example
the delayed reward in reinforcement learning settings. Credit assignment
to prior actions in the face of delayed reward is a notoriously difficult
task, and this remains so with humans in the loop. Knowledge of the lag
helps to assign credit appropriately to prior actions, and the
public health setting is no exception.



%The observed lag of
%\math{k=????} is well inside the deep-blue
%region in Figure~\ref{fig:model2}.

\paragraph{Acknowledgments.}
We thank Abhijit Patel, Sibel Adali and Zainab Magdon-Ismail for
provoking discussions on this topic.




==> macros <==
\def\mvec#1#2{[#1_1,\ldots ,#1_#2]}
\def\msum#1#2#3{$$\sm_{#1=#2}^#3$$}
\def\mint#1#2{$$\int_#1^#2$$}
\def\math#1{$#1$}
\def\mathd#1{$$#1\eqa$$}
\def\mand#1{$$#1$$}
\def\v#1{{\mathbf #1}}
\def\frac#1#2{{#1\over #2}}
\def\ital#1{{\it #1}}
\def\mld#1{\begin{equation}
#1
\end{equation}}
\def\eqar#1{\begin{eqnarray}
#1
\end{eqnarray}}
\def\eqan#1{\begin{eqnarray*}
#1
\end{eqnarray*}}

\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareMathSymbol{\N}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\Z}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\R}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\Q}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\I}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\C}{\mathbin}{AMSb}{"43}

%\def\R{{\mathbf R\hspace*{-1.65ex}\rule{0.08ex}{1.35ex}\hspace*{1.65ex}}} 
\def\Nat{{\mathbf N\hspace*{-1.89ex}\rule{0.07ex}{1.5ex}\hspace*{1.89ex}\hspace*{-1.7ex}\rule{0.1ex}{1.5ex}\hspace*{1.7ex}\hspace*{-.6ex}\rule{0.1ex}{1.5ex}\hspace*{.6ex}}}
%\def\Q{{\mathbf Q\hspace*{-1.35ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.4ex}}}
%\def\C{{\mathbf C\hspace*{-1.25ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.25ex}}}
\def\qed{\hfill\rule{2mm}{2mm}}
\def\sm{\sum\limits}
\def\choose#1#2{\left({{#1}\atop{#2}}\right)}
\def\cl#1{{\cal #1}}
\def\prob#1{{P\left[{#1}\right]}}
%\def\implies{\Rightarrow}
\def\mathbox#1{{\fbox{\math{#1}}}}
\def\mandbox#1{{\fbox{\math{\displaystyle #1}}}}
\def\argmin{\mathop{\hbox{argmin}}\limits}
\def\argmax{\mathop{\hbox{argmax}}\limits}

\def\mbf#1{{\mbox{\boldmath{$#1$}}}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
%\def\Z{{\mathbf Z}}
\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\exp#1{{\left\langle#1\right\rangle}}
\def\E#1{{{\mathbf E}\left[#1\right]}}
%\def\mod#1{{\left|#1\right|}}
\def\norm#1{{|\!|\,#1\,|\!|}}
\def\floor#1{{\left\lfloor\,#1\,\right\rfloor}}
\def\ceil#1{{\left\lceil\,#1\,\right\rceil}}
\def\r#1{{(\ref{#1})}}
\def\rot#1{{\rotatebox{90}{#1\ }}}

\newtheorem{theorem}{\bf Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{axiom}[theorem]{Axiom}


%%%%


\newcommand{\mychapter}[1]{\setcounter{exercisenum}{1}\chapter{#1}}
\newcommand{\mysection}[1]{\setcounter{exercisenum}{1}\section{#1}}
\newcounter{exercisenum}

\newenvironment{exercise}{
\  

\vskip 0.15in
\hrule height0.5pt
\begin{quote}{\bf Exercise \thesection.\theexercisenum}
\addtocounter{exercisenum}{1}
%\begin{spacing}{1}

\medskip
\sf \small

}
{
%\end{spacing}
\end{quote}
\hrule height0.5pt

\bigskip
\noindent}


%%%%

\newenvironment{algocode}{
\begin{center}
\begin{minipage}{4in}
\begin{algorithmic}
}
{
\end{algorithmic}
\end{minipage}
\end{center}
}


\newenvironment{algocode_num}[1]{
\begin{center}
\begin{minipage}{4in}
\begin{algorithmic}[#1]
}
{
\end{algorithmic}
\end{minipage}
\end{center}
}


\newenvironment{functioncode}[1]{
\begin{center}\begin{minipage}{4in}
#1\{
\begin{algorithmic}
}
{\end{algorithmic}
\}
\end{minipage}
\end{center}}


\newenvironment{functioncode_num}[2]{
\begin{center}\begin{minipage}{4in}
#1\{
\begin{algorithmic}[#2]
}
{\end{algorithmic}
\}
\end{minipage}
\end{center}}


%%%%




\newenvironment{problem}{
\  

\vskip 0.15in
\hrule height1pt
\begin{quote}{\bf Problem \thesection.\theexercisenum}
\addtocounter{exercisenum}{1}
%\begin{spacing}{1}

\medskip

}
{
%\end{spacing}
\end{quote}
\hrule height1pt

\bigskip
\noindent}


%%%%

\newenvironment{example}[1]{
\begin{quotation}
\noindent {\bf Example{#1}:}
}
{
\end{quotation}
\noindent}

%%%%


%%%%
\newenvironment{tech}{
\begin{quote}
\hrule height2pt
\noindent {\bf Technical Point}
\begin{spacing}{1}

\medskip

}
{
\end{spacing}
\end{quote}
\hrule height2pt

\medskip

\noindent}

%%%%

\newenvironment{aside}{
\begin{quote}
\hrule height2pt
\noindent {\bf Side Point}
\begin{spacing}{1}

\medskip

}
{
\end{spacing}
\end{quote}
\hrule height2pt

\medskip

\noindent}

%%%%

\newenvironment{technote}{
\begin{quote}
\hrule height2pt
\noindent {\bf Technical Note}
\begin{spacing}{1}

\medskip

}
{
\end{spacing}
\end{quote}
\hrule height2pt

\medskip

\noindent}

%%%%

\newenvironment{techaside}{
\begin{quote}
\hrule height2pt
\noindent {\bf Technical Aside}
\begin{spacing}{1}

\medskip

}
{
\end{spacing}
\end{quote}
\hrule height2pt

\medskip

\noindent}

\newenvironment{probstat}[1]{
\begin{quote}
\noindent {\bf Problem #1:}
\begin{spacing}{1}

\medskip

}
{
\end{spacing}
\end{quote}
\noindent}

\newcommand{\stitle}[1]{\begin{center}{\bf\color[named]{Red}#1}\\[-.8em]\rule{\li
newidth}{1pt}\end{center}}
\newcommand{\myv}[1]{{ \bf #1} }
\newcommand{\mym}[1]{{ \bf #1} }
\newcommand{\red}[1]{{\color[named]{Red} #1}}
\newcommand{\blue}[1]{{\color[named]{Blue} #1}}


\def\qn#1{{{#1}?\hfill\bf\math{\bigcirc} 1\qquad\math{\bigcirc} 2\qquad\math{\bigcirc} 3\qquad\math{\bigcirc} 4\qquad\math{\bigcirc} 5}}

\def\dotfil{\leaders\hbox to 1.5mm{.}\hfill}
\newcounter{rmnum}
%\def\RN#1{\count0=#1\uppercase\expandafter{\romannumeral\count0}}
\def\RN#1{\setcounter{rmnum}{#1}\uppercase\expandafter{\romannumeral\value{rmnum}}}
\def\rn#1{\setcounter{rmnum}{#1}\expandafter{\romannumeral\value{rmnum}}}
\def\lequal{{\buildrel{\scriptscriptstyle <}\over{\scriptscriptstyle =}}}
\def\gequal{\ {\buildrel{\scriptstyle >}\over{\scriptstyle =}}\ }
\def\econd#1#2{\ {\buildrel{\scriptstyle #1}\over{\scriptstyle #2}}\ }

\def\smileyface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0){\spline(2,2.5)(4.7,0)(7,2.5)}
\end{picture}
}}
\def\sadface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0.5){\spline(2.5,0)(5,2.5)(7.5,0)}
\end{picture}
}}

\newcommand{\qedsymb}{\hfill{\rule{2mm}{2mm}}}
\newenvironment{proof}{\begin{trivlist}
\item[\hspace{\labelsep}{\bf\noindent Proof: }]}{\qedsymb\end{trivlist}}


==> macros_short <==
\def\mvec#1#2{[#1_1,\ldots ,#1_#2]}
\def\msum#1#2#3{$$\sm_{#1=#2}^#3$$}
\def\mint#1#2{$$\int_#1^#2$$}
\def\math#1{$#1$}
\def\mathd#1{$$#1\eqa$$}
\def\mand#1{$$#1$$}
\def\v#1{{\mathbf #1}}
\def\frac#1#2{{#1\over #2}}
\def\ital#1{{\it #1}}
\def\mld#1{\begin{equation}
#1
\end{equation}}
\def\eqar#1{\begin{eqnarray}
#1
\end{eqnarray}}
\def\eqan#1{\begin{eqnarray*}
#1
\end{eqnarray*}}

\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareMathSymbol{\N}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\Z}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\R}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\Q}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\I}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\C}{\mathbin}{AMSb}{"43}

%\def\R{{\mathbf R\hspace*{-1.65ex}\rule{0.08ex}{1.35ex}\hspace*{1.65ex}}} 
\def\Nat{{\mathbf N\hspace*{-1.89ex}\rule{0.07ex}{1.5ex}\hspace*{1.89ex}\hspace*{-1.7ex}\rule{0.1ex}{1.5ex}\hspace*{1.7ex}\hspace*{-.6ex}\rule{0.1ex}{1.5ex}\hspace*{.6ex}}}
%\def\Q{{\mathbf Q\hspace*{-1.35ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.4ex}}}
%\def\C{{\mathbf C\hspace*{-1.25ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.25ex}}}
\def\qed{\hfill\rule{2mm}{2mm}}
\def\sm{\sum\limits}
\def\choose#1#2{\left({{#1}\atop{#2}}\right)}
\def\cl#1{{\cal #1}}
\def\prob#1{{P\left[{#1}\right]}}
%\def\implies{\Rightarrow}
\def\mathbox#1{{\fbox{\math{#1}}}}
\def\mandbox#1{{\fbox{\math{\displaystyle #1}}}}
\def\argmin{\mathop{\hbox{argmin}}\limits}
\def\argmax{\mathop{\hbox{argmax}}\limits}

\def\mbf#1{{\mbox{\boldmath{$#1$}}}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
%\def\Z{{\mathbf Z}}
\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\exp#1{{\left\langle#1\right\rangle}}
\def\E#1{{{\mathbf E}\left[#1\right]}}
%\def\mod#1{{\left|#1\right|}}
\def\norm#1{{|\!|\,#1\,|\!|}}
\def\floor#1{{\left\lfloor\,#1\,\right\rfloor}}
\def\ceil#1{{\left\lceil\,#1\,\right\rceil}}
\def\r#1{{(\ref{#1})}}
\def\rot#1{{\rotatebox{90}{#1\ }}}

\newcommand{\stitle}[1]{\begin{center}{\bf\color[named]{Red}#1}\\[-.8em]\rule{\li
newidth}{1pt}\end{center}}
\newcommand{\myv}[1]{{ \bf #1} }
\newcommand{\mym}[1]{{ \bf #1} }
\newcommand{\red}[1]{{\color[named]{Red} #1}}
\newcommand{\blue}[1]{{\color[named]{Blue} #1}}
\newcommand{\green}[1]{{\color[named]{Green} #1}}
\newcommand{\light}[1]{{\color[rgb]{0.7,0.7,0.7} #1}}
\newcommand{\dark}[1]{{\color[rgb]{0,0,0} #1}}


\def\qn#1{{{#1}?\hfill\bf\math{\bigcirc} 1\qquad\math{\bigcirc} 2\qquad\math{\bigcirc} 3\qquad\math{\bigcirc} 4\qquad\math{\bigcirc} 5}}

\def\dotfil{\leaders\hbox to 1.5mm{.}\hfill}
\newcounter{rmnum}
%\def\RN#1{\count0=#1\uppercase\expandafter{\romannumeral\count0}}
\def\RN#1{\setcounter{rmnum}{#1}\uppercase\expandafter{\romannumeral\value{rmnum}}}
\def\rn#1{\setcounter{rmnum}{#1}\expandafter{\romannumeral\value{rmnum}}}
\def\lequal{{\buildrel{\scriptscriptstyle <}\over{\scriptscriptstyle =}}}
\def\gequal{\ {\buildrel{\scriptstyle >}\over{\scriptstyle =}}\ }
\def\econd#1#2{\ {\buildrel{\scriptstyle #1}\over{\scriptstyle #2}}\ }

\def\smileyface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0){\spline(2,2.5)(4.7,0)(7,2.5)}
\end{picture}
}}
\def\sadface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0.5){\spline(2.5,0)(5,2.5)(7.5,0)}
\end{picture}
}}

















==> macros_short.tex <==
\def\mvec#1#2{[#1_1,\ldots ,#1_#2]}
\def\msum#1#2#3{$$\sm_{#1=#2}^#3$$}
\def\mint#1#2{$$\int_#1^#2$$}
\def\math#1{$#1$}
\def\mathd#1{$$#1\eqa$$}
\def\mand#1{$$#1$$}
\def\v#1{{\mathbf #1}}
\def\frac#1#2{{#1\over #2}}
\def\ital#1{{\it #1}}
\def\mld#1{\begin{equation}
#1
\end{equation}}
\def\eqar#1{\begin{eqnarray}
#1
\end{eqnarray}}
\def\eqan#1{\begin{eqnarray*}
#1
\end{eqnarray*}}

\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareMathSymbol{\N}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\Z}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\R}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\Q}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\I}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\C}{\mathbin}{AMSb}{"43}

%\def\R{{\mathbf R\hspace*{-1.65ex}\rule{0.08ex}{1.35ex}\hspace*{1.65ex}}} 
\def\Nat{{\mathbf N\hspace*{-1.89ex}\rule{0.07ex}{1.5ex}\hspace*{1.89ex}\hspace*{-1.7ex}\rule{0.1ex}{1.5ex}\hspace*{1.7ex}\hspace*{-.6ex}\rule{0.1ex}{1.5ex}\hspace*{.6ex}}}
%\def\Q{{\mathbf Q\hspace*{-1.35ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.4ex}}}
%\def\C{{\mathbf C\hspace*{-1.25ex}\raise.15ex\hbox{\rule{0.095ex}{1.35ex}}\hspace*{1.25ex}}}
\def\qed{\hfill\rule{2mm}{2mm}}
\def\sm{\sum\limits}
\def\choose#1#2{\left({{#1}\atop{#2}}\right)}
\def\cl#1{{\cal #1}}
\def\prob#1{{P\left[{#1}\right]}}
%\def\implies{\Rightarrow}
\def\mathbox#1{{\fbox{\math{#1}}}}
\def\mandbox#1{{\fbox{\math{\displaystyle #1}}}}
\def\argmin{\mathop{\hbox{argmin}}\limits}
\def\argmax{\mathop{\hbox{argmax}}\limits}

\def\mbf#1{{\mbox{\boldmath{$#1$}}}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
%\def\Z{{\mathbf Z}}
\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\exp#1{{\left\langle#1\right\rangle}}
\def\E#1{{{\mathbf E}\left[#1\right]}}
%\def\mod#1{{\left|#1\right|}}
\def\norm#1{{|\!|\,#1\,|\!|}}
\def\floor#1{{\left\lfloor\,#1\,\right\rfloor}}
\def\ceil#1{{\left\lceil\,#1\,\right\rceil}}
\def\r#1{{(\ref{#1})}}
\def\rot#1{{\rotatebox{90}{#1\ }}}

\newcommand{\stitle}[1]{\begin{center}{\bf\color[named]{Red}#1}\\[-.8em]\rule{\li
newidth}{1pt}\end{center}}
\newcommand{\myv}[1]{{ \bf #1} }
\newcommand{\mym}[1]{{ \bf #1} }
\newcommand{\red}[1]{{\color[named]{Red} #1}}
\newcommand{\blue}[1]{{\color[named]{Blue} #1}}
\newcommand{\green}[1]{{\color[named]{Green} #1}}
\newcommand{\light}[1]{{\color[rgb]{0.7,0.7,0.7} #1}}
\newcommand{\dark}[1]{{\color[rgb]{0,0,0} #1}}


\def\qn#1{{{#1}?\hfill\bf\math{\bigcirc} 1\qquad\math{\bigcirc} 2\qquad\math{\bigcirc} 3\qquad\math{\bigcirc} 4\qquad\math{\bigcirc} 5}}

\def\dotfil{\leaders\hbox to 1.5mm{.}\hfill}
\newcounter{rmnum}
%\def\RN#1{\count0=#1\uppercase\expandafter{\romannumeral\count0}}
\def\RN#1{\setcounter{rmnum}{#1}\uppercase\expandafter{\romannumeral\value{rmnum}}}
\def\rn#1{\setcounter{rmnum}{#1}\expandafter{\romannumeral\value{rmnum}}}
\def\lequal{{\buildrel{\scriptscriptstyle <}\over{\scriptscriptstyle =}}}
\def\gequal{\ {\buildrel{\scriptstyle >}\over{\scriptstyle =}}\ }
\def\econd#1#2{\ {\buildrel{\scriptstyle #1}\over{\scriptstyle #2}}\ }

\def\smileyface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0){\spline(2,2.5)(4.7,0)(7,2.5)}
\end{picture}
}}
\def\sadface{{
\begin{picture}(13,13)
\allinethickness{1.5pt}
\put(6.5,3.5){\circle{13}} 
\put(3.9,5.5){\circle*{1.25}} 
\put(8.7,5.5){\circle*{1.25}}
\put(1.7,0.5){\spline(2.5,0)(5,2.5)(7.5,0)}
\end{picture}
}}
















